Labrador: Exploring the Limits of Masked Language Modeling for Laboratory Data

In this work we introduce Labrador, a pre-trained Transformer model for laboratory data. Labrador and BERT were pre-trained on a corpus of 100 million lab test results from electronic health records (EHRs) and evaluated on various downstream outcome prediction tasks. Both models demonstrate mastery of the pre-training task but neither consistently outperform XGBoost on downstream supervised tasks. Our ablation studies reveal that transfer learning shows limited effectiveness for BERT and achieves marginal success with Labrador. We explore the reasons for the failure of transfer learning and suggest that the data generating process underlying each patient cannot be characterized sufficiently using labs alone, among other factors. We encourage future work to focus on joint modeling of multiple EHR data categories and to include tree-based baselines in their evaluations.

==> sections/author_contributions.tex <==
BK helped write the UMAP code and the manuscript, CW helped write the fine-tuning
experiment code, DB wrote the remaining code and conducted the
experiments present in the paper, and AB helped oversee the project and
conceive of the original idea. Correspondence to David Bellamy.

==> sections/contributions.tex <==
\subsection*{Generalizable Insights about Machine Learning in the Context of Healthcare}

\begin{itemize}
\item
  We design a novel Transformer architecture, \labrador, that can be pre-trained on (integer, float) data in a truly continuous manner and show that it outperforms BERT.
\item We provide a convenient method to tokenize EHR datasets that include a mixture of categorical and continuous data using the empirical cumulative distribution function (eCDF) of each continuous feature.
\item
  We demonstrate that MLM pre-training on MIMIC-IV data does not
  transfer well to downstream outcome prediction tasks and discuss the implications for future pre-training work with lab data.
\item
  We provide key future directions for self-supervised pre-training on structured EHR data.
\item
  We open-source our outcome prediction evaluation datasets, model weights and code so that future work can be benchmarked against our results.
\end{itemize}

==> sections/thanks.tex <==
DB would like to thank Dr. Tianxi Cai for her insightful idea
to transform the lab values using their empirical CDF. We also thank Dr.
Leo Celi for his help teaching us about the invaluable MIMIC dataset and the importance of advancing this work.
